Bridging the Data Provenance Gap Across Text, Speech and Video

Progress in AI is driven largely by the scale and quality of training data. Despite this, there is a deficit of empirical analysis examining the attributes of well-established datasets beyond text. In this work we conduct the largest and first-of-its-kind longitudinal audit across modalities--popular text, speech, and video datasets--from their detailed sourcing trends and use restrictions to their geographical and linguistic representation. Our manual analysis covers nearly 4000 public datasets between 1990-2024, spanning 608 languages, 798 sources, 659 organizations, and 67 countries. We find that multimodal machine learning applications have overwhelmingly turned to web-crawled, synthetic, and social media platforms, such as YouTube, for their training sets, eclipsing all other sources since 2019. Secondly, tracing the chain of dataset derivations we find that while less than 33% of datasets are restrictively licensed, over 80% of the source content in widely-used text, speech, and video datasets, carry non-commercial restrictions. Finally, counter to the rising number of languages and geographies represented in public AI training datasets, our audit demonstrates measures of relative geographical and multilingual representation have failed to significantly improve their coverage since 2013. We believe the breadth of our audit enables us to empirically examine trends in data sourcing, restrictions, and Western-centricity at an ecosystem-level, and that visibility into these questions are essential to progress in responsible AI. As a contribution to ongoing improvements in dataset transparency and responsible use, we release our entire multimodal audit, allowing practitioners to trace data provenance across text, speech, and video.

==> tables/collection.tex <==
\begin{table*}[t!]
\centering
% \footnotesize
\renewcommand{\arraystretch}{1.5}
\begin{adjustbox}{width=\textwidth}
\begin{tabular}{p{3cm} | p{16cm}}
\toprule
\textsc{Attribute} & \textsc{Details}  \\
\midrule

\textbf{Aggregator Links} & Instances of the dataset on GitHub, HuggingFace, Papers with Code, ArXiv, and Semantic Scholar are manually linked. This allows artifact, usage, and licensing metadata to be cross-referenced. \\ \rowcolor[gray]{0.9}
\textbf{Sources} & The original sources from which the data was collected. This includes websites or databases, human annotation, and model-generated content, wherever disclosed.  \\
\textbf{Licenses} & The dataset licenses and license URLs found on associated GitHub, HuggingFace, website, and academic paper pages. We also use \citet{longpre2023data} guidelines to classify licenses by use type (non-commercial, unspecified, all uses permitted), attribution, and copyleft restrictions.  \\ \rowcolor[gray]{0.9}
\textbf{Creators} & The organizations attributed with curating the dataset (not the underlying data). These organizations are categorized by country and by industry vs academia.  \\
\textbf{Tasks} & The specific tasks associated with the supervised datasets.  \\ \rowcolor[gray]{0.9}
\textbf{Size Metrics} & The size of the dataset, measured in dialog turns and tokens for text, the number of hours for video and speech, as well as the number of speakers for speech.  \\
% \midrule
\textbf{Languages} & The languages and language families represented in the text or speech. \\


\bottomrule
\end{tabular}
\end{adjustbox}
% \captionsetup{justification=centering}
\caption{The \textbf{list of dataset attributes}, their collection process, and the modalities they were collected for (includes only attributes with 2+ modalities). All attributes are manually collected. Annotation guidelines are available in \cref{app:attribute-annotation}.}
\label{tab:attributes}
\vspace{-2mm}
\end{table*}


